Kernel machines that adapt to GPUs for effective large batch training

Modern machine learning models are typically trained using Stochastic Gradient Descent (SGD) on massively parallel computing resources such as GPUs. Increasing mini-batch size is a simple and direct way to utilize the parallel computing capacity. For small batch an increase in batch size results in the proportional reduction in the training time, a phenomenon known as linear scaling. However, increasing batch size beyond a certain value leads to no further improvement in training time. In this paper we develop the first analytical framework that extends linear scaling to match the parallel computing capacity of a resource. The framework is designed for a class of classical kernel machines. It automatically modifies a standard kernel machine to output a mathematically equivalent prediction function, yet allowing for extended linear scaling, i.e., higher effective parallelization and faster training time on given hardware. The resulting algorithms are accurate, principled and very fast. For example, using a single Titan Xp GPU, training on ImageNet with $1.3\times 10^6$ data points and $1000$ labels takes under an hour, while smaller datasets, such as MNIST, take seconds. As the parameters are chosen analytically, based on the theoretical bounds, little tuning beyond selecting the kernel and the kernel parameter is needed, further facilitating the practical use of these methods.

==> app.tex <==
\section{Experimental Setup}
\label{app:expr-setup}
\noindent {\bf Computing Resource.} All experiments were run on a single workstation equipped with 128GB main memory, two Intel Xeon(R) E5-2620 processors, and one Nvidia GTX Titan Xp (Pascal) GPU.


\begin{wraptable}{r}{8.5cm}
\centering
\vspace{-4mm}
\begin{adjustbox}{center}
\resizebox{8.5cm}{!}{
\begin{tabular}{|l||c|c|c|}
\hline
Dataset & $n$ & $d$ & Label \\ \hline % & $\gamma^{\dagger}$ \\ \hline
CIFAR-10
& $5 \times 10^4$ & 1024 & \{0,...,9\} \\ \hline % & 2e-2 \\ \hline
MNIST
& $6 \times 10^4$ & 784 & \{0,...,9\} \\ \hline % & 2e-2 \\ \hline
SVHN
& $7 \times 10^4$ & 1024 & \{1,...,10\} \\ \hline % & 2e-2 \\ \hline
HINT-S
& $2 \times 10^5$ & 425 & $\{0,1\}^{64}$ \\ \hline % & 2e-3 \\ \hline
TIMIT
& $1.1 \times 10^6$ & 440 & \{0,...,143\} \\ \hline % & 3e-3 \\ \hline
20 Newsgroups
& $1.6 \times 10^4$ & 100 & $\{0,1\}^{20}$ \\ \hline % & 2e-2 \\ \hline
\end{tabular}
}
\end{adjustbox}
\vspace{-5mm}
\end{wraptable}
%%%%%%%%%%%%%%%%%%
\noindent {\bf Datasets.}
The table on the right summarizes
the datasets used in experiments.
We map multiclass labels to multiple binary labels (e.g. one label of $c$ classes to one $c$-length binary vector).
For image datasets including MNIST~\cite{lecun1998gradient}, CIFAR-10~\cite{krizhevsky2009learning}, and SVHN~\cite{netzer2011reading}, color images are first transformed to grayscale images. We then rescale the range of each feature to $[0, 1]$.
For HINT-S~\cite{healy2013algorithm} and TIMIT~\cite{garofolo1993darpa}, we normalize each feature by z-score. 
To efficiently fit the
20 Newsgroups~\cite{Lang95} dataset
with kernel regression, we transform its sparse feature vector (bag of words) into dense feature vector by summing up the corresponding embeddings of the words from~\cite{pennington2014glove}.


\noindent {\bf Hyperparameters.} For consistent comparison, all iterative methods use mini-batch of size $m = 256$.
The EigenPro preconditioner in~\cite{ma2017diving} is constructed using the top $k = 160$ eigenvectors of a subsampled training set of size $M = 5000$ (or the training set when its size is less than 5000).


\input{tbls/bandwidth.tex}
\noindent {\bf Kernel Bandwidth Selection.} For each dataset, we select the bandwidth $\sigma$ for Gaussian kernel $k(x, y) = \exp(-\frac{\norm{x - y}^2}{2\sigma^2})$ and Laplace kernel $k(x, y) = \exp(-\frac{\norm{x - y}}{\sigma})$ through cross-validation on a small subsampled dataset. The final bandwidths used for all datasets are listed in the table on the right side.


% \section{Supplementary Experimental Results}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{|c||c|c||c|c||c|c||c|c||}
% \hline
% \multirow{3}{*}{Label} & \multicolumn{8}{c|}{Size of subsample training data} \\ \cline{2-9} 
%  & \multicolumn{2}{c||}{$5 \cdot 10^3$} & \multicolumn{2}{c||}{$1.5 \cdot 10^4$} & \multicolumn{2}{c||}{$3 \cdot 10^4$} & \multicolumn{2}{c||}{$6 \cdot 10^4$} \\ \cline{2-9} 
%  & EiPro & SGD & EiPro & SGD & EiPro & SGD & EiPro & SGD \\ \hline

% Original & 2 & 75 & 3 & 129 & 4 & 141 & 4 & 151 \\ \hline

% Random & 4 & 112 & 4 & 131 & 7 & 181 & 7 & 184 \\ \hline

% \end{tabular}
% \caption{Epochs to overfit MNIST with original label and random label using EigenPro (EiPro) and SGD}
% \end{table}

% \input{figs/lc_synth_real.tex}


==> expr.tex <==
\section{Experimental Results}

\noindent {\bf .}
\newline

\noindent {\bf Comparisons to the state-of-the-art.}


==> figs/ep2-m-c.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
  \includegraphics[width=.6\textwidth]{figs/eigenpro_m_c_2.png}
    \vspace{-5mm}
	\caption{Faster convergence with adaptive kernel}
  \label{fig:train}
\end{wrapfigure}

==> tbls/sota.tex <==
\begin{minipage}{\textwidth}
% \caption{Comparison to large scale kernel results (Gaussian kernel)}
\label{tbl:sota}
\begin{threeparttable}
\begin{adjustbox}{center}
\resizebox{6in}{!}{
\begin{tabular}{|c|c||c|c|c|c|c|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Size} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}EigenPro\\ (use 1 GTX Titan Xp)\end{tabular}} & \multicolumn{3}{c|}{Other results} \\ \cline{3-7} \cline{3-7} 
 &  & error & GPU time & resource/time & error & reference \\ \hline \hline
MNIST & $1 \cdot 10^6$ & 0.67\% & \textbf{21 m} & \begin{tabular}[c]{@{}c@{}}1.1 h on\\ 1344 AWS vCPUs\end{tabular} & 0.72\% & PCG~\cite{avron2016faster} \\ \hline \hline
\multirow{5}{*}{TIMIT} & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}$1.1 \cdot 10^6$\\ / $2 \cdot 10^6$\end{tabular}} & \multirow{5}{*}{32.0\%} & \multirow{5}{*}{\textbf{15 m}} & \begin{tabular}[c]{@{}c@{}}multiple AWS\\ g2.2xlarge instances\end{tabular} & 32.4\% & DNN~\cite{may2017kernel} \\ \cline{5-7} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}7.5 h on \\ 1024 AWS vCPUs\end{tabular} & 33.5\% & BCD~\cite{tu2016large} \\ \cline{5-7} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}512 IBM\\ Blue Gene/Q cores\end{tabular} & 33.5\% & Ensemble~\cite{huang2014kernel} \\ \cline{5-7} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}1.5 h on\\ 1 Tesla K40c\end{tabular} & 32.3\% & Falkon~\cite{rudi2017falkon} \\ \cline{5-7} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}multiple AWS \\ g2.2xlarge instances\end{tabular} & 30.9\% & \begin{tabular}[c]{@{}c@{}}SparseKernel~\cite{may2017kernel}\\ (with learned features)\end{tabular} \\ \hline \hline
\multirow{2}{*}{SUSY} & \multirow{2}{*}{$4 \cdot 10^6$} & \multirow{2}{*}{19.7\%} & \multirow{2}{*}{\textbf{0.8 m}} & \begin{tabular}[c]{@{}c@{}}36 m on\\ IBM POWER8\end{tabular} & $\approx 20\%$ & Hierarchical~\cite{chen2016hierarchically} \\ \cline{5-7} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}4 m on\\ 1 Tesla K40c\end{tabular} & 19.6\% & Falkon~\cite{rudi2017falkon} \\ \hline
\end{tabular}
}
\end{adjustbox}
\end{threeparttable}
%\vspace{-6mm}
\end{minipage}
